Efficient Low-Rank Matrix Estimation, Experimental Design, and Arm-Set-Dependent Low-Rank Bandits

We study low-rank matrix trace regression and the related problem of low-rank matrix bandits. Assuming access to the distribution of the covariates, we propose a novel low-rank matrix estimation method called LowPopArt and provide its recovery guarantee that depends on a novel quantity denoted by B(Q) that characterizes the hardness of the problem, where Q is the covariance matrix of the measurement distribution. We show that our method can provide tighter recovery guarantees than classical nuclear norm penalized least squares (Koltchinskii et al., 2011) in several problems. To perform efficient estimation with a limited number of measurements from an arbitrarily given measurement set A, we also propose a novel experimental design criterion that minimizes B(Q) with computational efficiency. We leverage our novel estimator and design of experiments to derive two low-rank linear bandit algorithms for general arm sets that enjoy improved regret upper bounds. This improves over previous works on low-rank bandits, which make somewhat restrictive assumptions that the arm set is the unit ball or that an efficient exploration distribution is given. To our knowledge, our experimental design criterion is the first one tailored to low-rank matrix estimation beyond the naive reduction to linear regression, which can be of independent interest.

==> sections/analysis.tex <==
%subsection
\label{sec:analysis}

\paragraph{Analysis of Algorithm~\ref{alg:lowPopart}} 



The core part of explore-then-commit algorithm is the estimation error of the exploration phase. We proved the following estimation error guarantee:

\begin{theorem}\label{thm:lpopart}
Suppose that Algorithm \ref{alg:lowPopart} is run with action set $\cA$, sample size $n_0$, pilot estimator $\Theta_0$ and pilot estimation error bound $R_0$, such that  $\max_{A \in \cA} \abs{ \inner{\Theta_0 - \Theta}{A} } \leq R_0$, then its output $\hat{\Theta}$ is such that $\rank(\hat{\Theta}) \leq r$, and:  
    \begin{align}
        \| \hat{\Theta} -\Theta^*\|_{op}
        \leq 
        O\del{ 
        (\sigma+R_0)\sqrt{\frac{d}{n_0 \cC_{\min}}\ln \frac{2d}{\delta}}
        }~.
    \end{align}
\end{theorem}\label{thm:from Minsker}
\begin{proof}
    First, we recall the following lemma of \citet{minsker2018sub} on robust matrix mean estimation: 
    \begin{lemma}[Modification of Corollary 3.1, \citet{minsker2018sub}]
        For a sequence independent, identically distributed random matrix $M_i (i=1,\cdots, n)$, let 
        \kj{typo in the definition below?}
        $$\sigma_n^2 = \max\del{\sum_{i=1}^n \|\EE [M_i M_i^\top ]\|_{op}, \|\sum_{i=1}^n \EE [M_i^\top M_i]\|_{op}}$$
        Given $\nu=\frac{t\sqrt{n}}{\sigma_n^2}$, let $X_i = \phi (\nu \cH(M_i ))$ and let $\hat{T}=\frac{1}{n \nu} (\sum_{i=1}^n 
    X_i)_{12}$. Then, with probability at least $1-\delta$, we have
    
    \begin{align*}
        \| \hat{T} - \EE[M_i]\|_{op}\leq \frac{t}{\sqrt{n}}
    \end{align*}
    \end{lemma}
To utilize this Lemma \ref{thm:from Minsker}, we choose $M_i$'s so that
\begin{itemize}
    \item $\EE\sbr{M_i} = \Theta^* - \Theta_0$ so that $\hat{T}$ estimates the hidden parameter $\Theta^*-\Theta_0$
    \item $\sigma_{m}^2$ is well-controlled. 
\end{itemize}

It can be checked that $M_i = \reshape \del{Q(\pi^*)^{-1} (Y_i - \inner{\Theta_0}{X_i}) \vec(X_i)}$ satisfies the condition with $\sigma_{n}^{2} \leq 2(\sigma^2 + R_{0}^2) \frac{d n_0}{\cC_{\min}}$ (See Appendix \ref{Appendix: proof of main theorem} for the proof.) Substituting $\sigma_{n}^2$ to $2(\sigma^2 + R_{0}^2) \frac{d n_0}{\cC_{\min}}$, $t=\sqrt{\frac{2\sigma_n^2}{n_0}\ln \frac{2d}{\delta}}$ leads the desired result. 
Note that for all $j \geq r+1$, $\sigma_j(\Theta^*) = 0$.
    By Weyl's Theorem, for all $j \geq r+1$, we have that $\sigma_j(\Theta_1) \leq 2\sqrt{\frac{((\sigma^2 + R_{0}^2) )(d_1 + d_2) \del{\ln \frac{2(d_1 + d_2)}{\delta} } }{\cC_{\min}n_0}}$. As a consequence, $\hat{\Theta}$ has rank at most $r$, hence $\hat{\Theta} - \Theta^*$ has rank at most $2r$. 
    
    Moreover, by construction, $\| \hat{\Theta} - \Theta_1 \|_{\op} \leq 2\sqrt{\frac{(\sigma^2 + R_{0}^2) (d_1 + d_2) \del{ \ln \frac{2(d_1 + d_2)}{\delta} } }{\cC_{\min}n_0}}$. By triangle inequality, we have
    \[
    \| \hat{\Theta} - \Theta^* \|_{\op} 
    \leq 
    4\sqrt{\frac{ (\sigma^2 + R_{0}^2) (d_1 + d_2)\del{\ln \frac{2(d_1 +d_2)}{\delta} } }{\cC_{\min}n_0}}
    \qedhere
    \]
\end{proof}


\begin{remark}
A alternative and popular approach for matrix estimation is nuclear norm penalized least squares~\citep{tsybakov2011nuclear}, which also yields a strong recovery guarantee of $\| \hat{\Theta} - \Theta^* \|_F \leq \tilde{O}(\sqrt{ \frac{r }{n C_{\min}^2} })$ and $\| \hat{\Theta} - \Theta^* \|_* \leq \tilde{O}(\sqrt{ \frac{r^2}{n C_{\min}^2} })$.
However, we show in Appendix~\ref{Appendix:comparison with Tsybakov} that under Assumption~\ref{assumption:op-bound}, $C_{\min} \leq \frac1d$, and as a consequence, the guarantees of nuclear norm penalized least squares is weaker than that of $\lpopart$.
\end{remark}

%However, we have taken a step further here by incorporating the design of experiment and utilizing estimation of \citet{minsker2018sub} instead. As a result, we have successfully reduced the order of $\cC_{\min}^{-1}$ from $1$ to $1/2$. For more details, please refer to the Appendix  


A naive application of $\textsf{LowPopArt}$ with pilot estimator $0_{d_1 \times d_2}$ gives an estimator $\hat{\Theta}$ such that  
$\| \hat{\Theta} -\Theta^*\|_{op}
\leq 
\tilde{O}\del{ (\sigma + S_*)
\sqrt{\frac{d}{n_0 \cC_{\min}}}}$; the dependence on $S_*$ is somewhat undesirable when $S_* \gg \sigma$.
Motivated by this, we propose a bootstrapped version of $\textsf{LowPopArt}$ whose estimation error guarantee is $\tilde{O}\del{ \sigma
\sqrt{\frac{d}{n_0 \cC_{\min}}}}$ under mild assumptions, i.e. $\textsf{Warm-LowPopArt}$ (Algorithm~\ref{alg:warm-popart}). 
Its key idea is to first construct a coarse estimator $\Theta_0$ such that $\| \Theta_0 - \Theta^* \|_{\op} \leq \sigma$, which ensures that $\max_{A \in \cA} \abs{ \inner{\Theta_0 - \Theta^*}{A} } \leq \sigma$; it subsequently uses $\Theta_0$ as a pilot estimator to obtain the final estimate $\hat{\Theta}$. 
Formally, we have the following theorem:


%An somewhat undesirable property of $\mathsf{LowPopArt}$'s guarantee is its dependency on the range


%\ln \frac{2d}{\delta}}




\begin{algorithm}
\caption{$\textsf{Warm-LowPopArt}$: a bootstrapped version of $\mathsf{LowPopArt}$}
\label{alg:warm-popart}

\begin{algorithmic}[1]
\STATE Input: action set $\cA$, sample size $n_0$, failure rate $\delta$. 

\STATE $\Theta_0 \gets \mathsf{LowPopArt} (\cA, n_0/2, 0_{d_1 \times d_2}, S_*,  \delta/2)$

\STATE $\hat{\Theta} \gets \mathsf{LowPopArt} (\cA, n_0/2, \Theta_0, \sigma, \delta/2)$

\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:wlpopart}
Suppose that Algorithm \ref{alg:warm-popart} is run with action set $\cA$, sample size $n_0$, failure rate $\delta$, such that  $\max_{A \in \cA} \abs{ \inner{\Theta_0 - \Theta}{A} } \leq R_0$, 
and $n_0 \geq \tilde{O}\del{ \frac{d}{C_{\min}} \cdot (\frac{\sigma + S_*}{\sigma})^2 }$,
then its output $\hat{\Theta}$ is such that $\rank(\hat{\Theta}) \leq r$, and:  
    \begin{align}
        \| \hat{\Theta} -\Theta^*\|_{op}
        \leq 
        O(\sigma
        \sqrt{\frac{2d}{n_0 \cC_{\min}}\ln \frac{2d}{\delta}})
    \end{align}
\end{theorem}\label{thm:from Minsker}


%and pilot estimation error bound $R_0$, such that  $\max_{A \in \cA} \abs{ \inner{\Theta_0 - \Theta}{A} } \leq R_0$. 


==> sections/def-kjun-v4a.tex <==

%_ better math font
\usepackage{amsthm,amsmath,bbm,amsfonts,amssymb}
\usepackage{dsfont} % require for using \mathds{1}
\usepackage{mathtools}
\usepackage{commath}
\mathtoolsset{showonlyrefs=false}

\usepackage{xspace}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
%\usepackage[usenames,dvipsnames]{xcolor} % for color names


\usepackage{hyperref,url}
\usepackage{cleveref} % must be loaded after amsthm

\usepackage[usenames,dvipsnames]{xcolor} % for color names

\usepackage{wrapfig}
\usepackage[export]{adjustbox}
\def\imagetop#1{\vtop{\null\hbox{#1}}} % adjusting location of box in table
%- synctex
\synctex=1
% \pdfoutput=1  % for arxiv submission

% For algorithms

%\usepackage{algorithm}
%\usepackage{algorithmic}

\usepackage{graphicx,tabularx}
\usepackage{multirow,hhline}% http://ctan.org/pkg/multirow
\usepackage{booktabs}% to use \midrule for drawing a horizontal line in align environment

\usepackage{capt-of}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\usepackage{enumitem}

\allowdisplaybreaks % This allows breaking multi-line equations

\usepackage{pbox} % new line in a table cell -- http://tex.stackexchange.com/questions/2441/how-to-add-a-forced-line-break-inside-a-table-cell


%--- prints out an error when the symbol is already defined.
\def\safedef#1{% 
   \ifx#1\undefined
      \expandafter\def\expandafter#1%
   \else
      \errmessage{The \string#1 is defined already}% 
      \expandafter\def\expandafter\tmp
   \fi
}



% for vertical alignment of includegraphics
%- http://tex.stackexchange.com/questions/101858/make-two-figures-aligned-at-top
\usepackage[export]{adjustbox}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\cm}{\ding{51}}%
\newcommand{\gyes}{{\color[rgb]{0,.8,0}\cmark}}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\xm}{\ding{55}}%
\newcommand{\rno}{{\color[rgb]{.8,0,0}\xmark}}

% define your comment color here
\newcommand{\jerry}[1]{{ \color[cmyk]{0,0.61,0.87,0}jerry: #1 }}
\newcommand{\rob}[1]{{ \color[rgb]{0,0.718,0.179}rob: #1 }}
\newcommand{\kwang}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}
\newcommand{\kw}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}

\newcommand{\kj}[1]{{\color{Orange}[KJ: #1]}}
\newcommand{\ks}[1]{{\color{OliveGreen}Kyoungseok: #1}}
\newcommand{\chicheng}[1]{{\color{blue}Chicheng: #1}}
\newcommand{\gray}[1]{{ \color[rgb]{.6,.6,.6} #1 }}
\newcommand{\blue}[1]{{\color[rgb]{.3,.5,1}#1}}
\newcommand{\grn}[1]{{\color{ForestGreen}#1}}
\newcommand{\org}[1]{{\color{Orange}#1}}
\newcommand{\vio}[1]{{\color{Violet}#1}}
\newcommand{\red}[1]{{\color[rgb]{1,.1,.1}#1}}
\newcommand{\gr}[1]{{\color[rgb]{.8,.8,.8}#1}}



%---------- setup theorem environment
\usepackage{framed}
\usepackage[most]{tcolorbox}
\definecolor{kjgray}{rgb}{.7,.7,.7}

\newtheoremstyle{kjstyle}
{1ex} % Space above
{\topsep} % Space below
{\itshape} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')

\newtheoremstyle{kjstylenoitalic}
{1ex} % Space above
{\topsep} % Space below
{} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')

\tcbset{kjboxstyle/.style={title={},breakable,colback=white,enhanced jigsaw,boxrule=1.3pt,sharp corners,colframe=kjgray,boxsep=0pt,coltitle={black},attach title to upper={},left=.8ex,bottom=.4em}}    
%    ,title after break={Lemma \thelemma\ (continued)}}
%}
%
%
\theoremstyle{kjstyle}\newtheorem{thm}{Theorem}
\AtBeginEnvironment{thm}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{thm}{\end{tcolorbox}}%
\theoremstyle{kjstyle}\newtheorem{lem}[thm]{Lemma}
\AtBeginEnvironment{lem}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{lem}{\end{tcolorbox}}%
\theoremstyle{kjstyle}\newtheorem{prop}[thm]{Proposition}
\AtBeginEnvironment{prop}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{prop}{\end{tcolorbox}}%
\theoremstyle{kjstyle}\newtheorem{cor}[thm]{Corollary}
\AtBeginEnvironment{cor}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{cor}{\end{tcolorbox}}%

\theoremstyle{kjstyle}\newtheorem{defn}{Definition}
\AtBeginEnvironment{defn}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{defn}{\end{tcolorbox}}%

\theoremstyle{kjstyle}\newtheorem{ass}{Assumption}
\AtBeginEnvironment{ass}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{ass}{\end{tcolorbox}}%
\renewcommand\theass{A\arabic{ass}}


\theoremstyle{kjstyle}\newtheorem{question}{Question}
\AtBeginEnvironment{question}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{question}{\end{tcolorbox}}%
% \renewcommand\theass{A\arabic{ass}}

% \theoremstyle{kjstylenoitalic}\newtheorem{remark}{Remark}
% \AtBeginEnvironment{remark}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{remark}{\end{tcolorbox}}%


%--------------- other ways to create box
\newcommand{\kjunboxold}[1]{\vspace{.5em}\\\fbox{%
    \begin{minipage}{\linewidth}
      \centering #1
    \end{minipage}%
  }\vspace{.5em}}
\def\lamp{\ensuremath{\lambda_\perp}}
\usepackage{mdframed}
\usepackage{lipsum}
\definecolor{kjgray}{rgb}{.7,.7,.7}
\makeatletter
\newcommand{\kjunbox}[1]{\vspace{.4ex}
  \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt]
    #1
  \end{mdframed}%
}
\makeatletter
\newcommand{\kjunboxcenter}[1]{\vspace{.4ex}
  \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt,userdefinedwidth=.8\linewidth,align=center]
    %[linecolor=black,innerleftmargin=.4em,innerrightmargin=.4em,userdefinedwidth=.8\linewidth,align=center]
    #1
  \end{mdframed}%
}
\makeatother


%--- to remove the space before paragraph : change 3.25ex to ...
\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0.8em \@plus 1ex \@minus .2ex}{-1em}%
  {\normalfont\normalsize\bfseries}%
}
\makeatother

%%- https://tex.stackexchange.com/questions/72692/highlight-an-equation-within-an-align-environment-with-color-option
%%------- this makes a border that covers other part of the equation....
%\usepackage[customcolors,shade]{hf-tikz} % after {}, (right, below) and then (left, above) offset... I don't know how it works; done by trial-and-error.
%\newcommand{\hll}[2]{\tikzmarkin[set fill color=yellow!30]{#1}(0.02,-.08)(-0.02,0.3)#2\tikzmarkend{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros for keeping track of symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%BEG-------- for list of symbols
\newcounter{textcnt}
%\newcommand\textlist{}
\newcommand\settext[2]{%
  \csgdef{text#1}{#2}}
\newcommand\addtext[1]{%
  \stepcounter{textcnt}%
  \csgdef{text\thetextcnt}{#1}}
\newcommand\gettext[1]{%
  \csuse{text#1}}
\newcommand\getcount{\thetextcnt}

\newcounter{colnum}
\newcommand\maketabularrow[1]{%
  \setcounter{colnum}{0}%
  \whileboolexpr
  { test {\ifnumcomp{\value{colnum}}{<}{#1}} }%
  {&\stepcounter{colnum}\thecolnum}
}

\newcounter{Jidx}
\newcommand\dsymhelper[2]{
  \addtext{\hyperlink{#1}{#2}}%
  \blue{\hypertarget{#1}{#2}}%
}
\newcommand\dsym[1]{
  \stepcounter{Jidx}
  \xdef\tmpname{Jsym.\theJidx}
  \expandafter\dsymhelper\expandafter{\tmpname}{#1}
} 
%END--------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
% \def\ddef#1{\expandafter\def\csname #1#1\endcsname{\ensuremath{\mathbb{#1}}}}
% \ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{{\boldsymbol{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSUVWXYZabcdeghijklmnopqrtsuvwxyz\ddefloop  % including f here causes icml21 style file to behave weird.
%\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{\mathbf{#1}}}}
%\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname h#1\endcsname{\ensuremath{\widehat{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrsuvwxyz\ddefloop % except for 't' because it is used by others
\def\ddef#1{\expandafter\def\csname hc#1\endcsname{\ensuremath{\widehat{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname t#1\endcsname{\ensuremath{\widetilde{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname r#1\endcsname{\ensuremath{\mathring{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname bar#1\endcsname{\ensuremath{\bar{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname wbar#1\endcsname{\ensuremath{\overline{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname tc#1\endcsname{\ensuremath{\widetilde{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop


\def\hmu{{\ensuremath{\hat{\mu}}} }
\def\bhmu{{\ensuremath{\boldsymbol{\hat{\mu}}} }}

\def\SS{{\mathbb{S}}}

\DeclareMathOperator*{\argmax}{arg~max}
\DeclareMathOperator*{\argmin}{arg~min}
\DeclareMathOperator{\EE}{\mathbb{E}}
\DeclareMathOperator{\VV}{\mathbb{V}}
\DeclareMathOperator{\PP}{\mathbb{P}}
\DeclareMathOperator{\hEE}{\hat{\mathbb{E}}}
\DeclareMathOperator{\one}{\mathds{1}\hspace{-.05em}}
\DeclareMathOperator{\Reg}{{\normalfont\text{Reg}}}
%\DeclareMathOperator*{\lap}{{\lessapprox}}
%\DeclareMathOperator*{\lapp}{{\lessapprox}}
\newcommand{\lap}{\mathop{}\!\lessapprox}
\newcommand{\lapp}{\mathop{}\!\lessapprox}
\newcommand{\gapp}{\mathop{}\!\gtrapprox}
\newcommand{\lsim}{\mathop{}\!\lesssim}
\newcommand{\gsim}{\mathop{}\!\gtrsim}


\def\RR{{\mathbb{R}}}
\def\NN{{\mathbb{N}}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\ubrace}[2]{{\underbrace{#1}_{\textstyle #2}}}
\newcommand{\sr}[2]{ {\mathop{}\stackrel{#1}{#2}}\mathop{}\, }
\newcommand*{\medcup}{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}}%
\newcommand*{\medcap}{\mathbin{\scalebox{1.5}{\ensuremath{\cap}}}}%
\def\bigmid{\,\middle|\,\xspace}
\newcommand{\fr}[2]{ { \frac{#1}{#2} }}
\def\lt{\left}
\def\rt{\right}
\def\suchthat{\ensuremath{\mbox{ s.t. }}} 
\def\dsum{\ensuremath{\displaystyle\sum}} 
\def\der{\ensuremath{\partial}\xspace}

\def\bbeta{{{\boldsymbol \beta}}}
\def\btheta{{{\boldsymbol \theta}}}
\def\bphi{{{\boldsymbol \phi}}}
\def\barbu{{\overline{\mathbf u}}}
\def\sign{\ensuremath{\text{sign}}}
\def\eps{\ensuremath{\epsilon}\xspace}
\def\hS{\ensuremath{\hat{S}}\xspace}

\def\larrow{\ensuremath{\leftarrow}\xspace} 
\def\rarrow{\ensuremath{\rightarrow}\xspace} 
\def\T{\ensuremath{\top}}  % transpose
\def\sig{\ensuremath{\sigma}\xspace}
\def\bsig{{\ensuremath{\boldsymbol{\sigma}}}}
\def\Pr{\ensuremath{\text{Pr}}} 
\def\eps{\ensuremath{\epsilon}\xspace}
\def\diag{\ensuremath{\text{\normalfont diag}}\xspace}
\def\supp{\ensuremath{\mbox{supp}}\xspace}
\def\decomp{\ensuremath{\mbox{decomp}}\xspace}

\def\balpha{{{\boldsymbol \alpha}}}
\def\bbeta{{{\boldsymbol \beta}}} % this causes error in section title
\def\btheta{{{\boldsymbol \theta}}} 
\def\bgamma{{{\boldsymbol \gamma}}} 
\def\hbtheta{{\widehat{\boldsymbol \theta}}} 
\def\bTheta{{{\boldsymbol \Theta}}} 
\def\bmu{{{\boldsymbol \mu}}}
\def\bpi{{\ensuremath{\bm{\pi}}\xspace}}  
\def\Dki{{\ensuremath{\Delta_{ki}}\xspace} }
\def\om{{\ensuremath{\omega}\xspace} }
\def\dt{{\ensuremath{\delta}\xspace} }
\def\sm{{\ensuremath{\setminus}\xspace} }

\def\grad{\ensuremath{\mathbf{\nabla}}\xspace}  

\def\bSigma{\ensuremath{\mathbf{\Sigma}}\xspace} 
\def\bLambda{\ensuremath{\boldsymbol{\Lambda}}\xspace} 
\def\hatbfP{\ensuremath{\widehat{\mathbf{P}}}\xspace} 
\def\hatbfpi{\ensuremath{\widehat{\boldsymbol{\pi}}}\xspace} 
\def\hatP{\ensuremath{\widehat{P}}\xspace} 
\def\hattheta{\ensuremath{\widehat{\theta}}\xspace} 
\def\hatQ{\ensuremath{\widehat{Q}}\xspace} 
\def\hatpi{\ensuremath{\widehat{\pi}}\xspace} 
\def\bftilpi{\ensuremath{\boldsymbol{\widetilde{\pi}}}\xspace} 
\def\bftilP{\ensuremath{\mathbf{\widetilde{P}}}\xspace} 
\def\bftilBeta{{\ensuremath{\boldsymbol{\widetilde{\beta}}}}\xspace} 
\def\tilpi{\ensuremath{\widetilde{\pi}}\xspace} 
\def\tilP{\ensuremath{\widetilde{P}}\xspace} 
\def\tilBeta{\ensuremath{\widetilde{\beta}}\xspace} 

\def\hatK{{\ensuremath{\widehat{K}}\xspace}} 
\def\hatT{{\ensuremath{\widehat{T}}\xspace}}
\def\hatW{{\ensuremath{\widehat{W}}\xspace}}
\def\hattau{{\ensuremath{\widehat{\tau}}\xspace}}
\def\sym{{\ensuremath{\text{Sym}}\xspace}} 

\def\logbar{{\ensuremath{\overline{\log}}}} 
\newcommand{\what}[1]{ {\ensuremath{\widehat{#1}}} }

\def\barT{\ensuremath{\overline{T}}\xspace} 
\def\bart{\ensuremath{\overline{t}}\xspace} 
\def\barV{\ensuremath{\overline{V}}\xspace} 
\def\barU{\ensuremath{\overline{U}}\xspace} 
\def\barG{\ensuremath{\overline{G}}} 
\def\barL{\ensuremath{\overline{L}}\xspace} 

\def\hatk{{\ensuremath{\what{k}}}\xspace}  
\def\ntil{\ensuremath{\tilde{n}}\xspace} 
\def\rtil{\ensuremath{\tilde{r}}\xspace} 
\def\hDelta{\ensuremath{\what{\Delta}}\xspace} 



%- ceiling and floor
\def\llfl{\left\lfloor} 
\def\rrfl{\right\rfloor}  
\def\llcl{\left\lceil}  
\def\rrcl{\right\rceil}  
\def\lfl{\lfloor} 
\def\rfl{\rfloor}  
\def\lcl{\lceil}  
\def\rcl{\rceil}  

%- pretty < and > symbol
\newcommand{\langl}{\begin{picture}(4.5,7)
\put(1.1,2.5){\rotatebox{60}{\line(1,0){5.5}}}
\put(1.1,2.5){\rotatebox{300}{\line(1,0){5.5}}}
\end{picture}}
\newcommand{\rangl}{\begin{picture}(4.5,7)
\put(.9,2.5){\rotatebox{120}{\line(1,0){5.5}}}
\put(.9,2.5){\rotatebox{240}{\line(1,0){5.5}}}
\end{picture}}

%- new on 20150826
\def\cmt{{\;//\;}}
\def\gam{{\ensuremath{\gamma}\xspace} }

%- new on 20151024
\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother

%- new on 20151123
\def\bl{{{\boldsymbol \ell}}}
\def\dsR{{{\mathds{R}}}}

%- new on 20160503
\def\cX{\ensuremath{\mathcal{X}}\xspace} 
\def\la{{\langle}}
\def\ra{{\rangle}}
\def\det{\ensuremath{\mbox{det}}}
\def\lam{\ensuremath{\lambda}}
\def\barV{\ensuremath{\overline{\mathbf{V}}}\xspace} 
\def\ibarV{\ensuremath{\overline{\mathbf{V}}^{-1}}\xspace} 
\def\iV{\ensuremath{{\mathbf{V}}^{-1}}\xspace} 
\def\hatth{\ensuremath{\widehat{\boldsymbol\theta}}\xspace} 
\def\tilth{\ensuremath{\tilde{\boldsymbol\theta}}\xspace} 
\def\barVinv{\ensuremath{\overline{\mathbf{V}}^{-1}}} 
\def\barVi{\ensuremath{\overline{\mathbf{V}}^{-1}}} 
\def\tilmu{{\ensuremath{\tilde{\mu}}\xspace} }

%- 20160705
\def\tiln{\ensuremath{\tilde{n}}\xspace} 

%- 20160728
\def\bell{{{\boldsymbol\ell}}}
\def\cC{\ensuremath{\mathcal{C}}\xspace} 
\def\cD{\ensuremath{\mathcal{D}}\xspace} 
\def\cW{\ensuremath{\mathcal{W}}\xspace} 
\def\cU{\ensuremath{\mathcal{U}}\xspace} 
\def\KL{\ensuremath{\normalfont{\mathsf{KL}}}}  

\def\l{{{\boldsymbol \ell}}}

%--- 20160829
\def\hatp{\ensuremath{\widehat p}}
\def\hatbfp{\ensuremath{\widehat{\mathbf{p}}}}
\def\tilg{\ensuremath{\widetilde{g}}}
\def\tilG{\ensuremath{\widetilde{G}}}
\def\tilbfg{\ensuremath{\widetilde{\mathbf{g}}}}
\def\bcI{\ensuremath{\boldsymbol{\mathcal{I}}}} 
\def\Active{\ensuremath{\text{Active}}}
\def\CBS{\ensuremath{\text{CBS}}}
\def\CBSE{\ensuremath{\text{CBSE}}}
\def\Regret{\ensuremath{\normalfont{\text{Regret}}}}
\def\Wealth{\ensuremath{\text{Wealth}}}
\def\CB{\ensuremath{\text{CB}}}

%--- 2016/09/16
\def\btau{\ensuremath{\boldsymbol{\tau}}\xspace} 
\newcommand{\wtil}[1]{ {\ensuremath{\widetilde{#1}}} }
\def\ccH{\ensuremath{c_\text{H}}}
\def\tH{\ensuremath{\text{H}}}
\def\bfeta{\ensuremath{\boldsymbol{\eta}}} 
\def\til{\widetilde} 
\def\vec{\text{vec}} 
\def\dsN{{{\mathds{N}}}}
\newcommand{\wbar}[1]{ {\ensuremath{\overline{#1}}} }
\def\barbeta{\wbar{\beta}}
\def\tilbeta{\tilde{\beta}}
\def\barC{\ensuremath{\wbar{C}}}
\def\tilC{\ensuremath{\wtil{C}}}
\def\barth{\ensuremath{\wbar{\theta}}\xspace} 

\def\dsR{\ensuremath{{\mathds R}}\xspace}
\def\hcalX{\ensuremath{\what{\mathcal X}}\xspace}
\def\hcalZ{\ensuremath{\what{\mathcal Z}}\xspace}
%\def\hth{\ensuremath{\what{\theta}}\xspace}
\def\bth{{{\boldsymbol \theta}}} 
\def\bfeta{{{\boldsymbol \eta}}} 
\def\hbth{{\what{\boldsymbol \theta}}} 
\def\hth{{\hat{ \theta}}} 
\def\bfUp{\ensuremath{\mathbf{U}_\perp}\xspace}
\def\Up{\ensuremath{\mathbf{U}_\perp}\xspace}
\def\lam{{\ensuremath{\lambda}\xspace} }
\def\bTheta{{{\boldsymbol \Theta}}}
\def\bTh{{{\boldsymbol \Theta}}}
\def\barbV{\ensuremath{\overline{\mathbf{V}}}\xspace} 

%- 20170228
\def\tL{\ensuremath{\mathbf{\text{L}}}}
\def\vec{\ensuremath{\text{vec}}}
\def\Th{{{\Theta}}} 
\def\Lam{{{{{\Lambda}}}}}
\def\bLam{{{{\boldsymbol{\Lambda}}}}}
\def\blam{{{\boldsymbol{{\lambda}}}}}
\def\bgam{{{\boldsymbol{{\gamma}}}}} 
\def\bom{{{\boldsymbol{{\omega}}}}} 
\def\lnorm{\left|\left|}
\def\rnorm{\right|\right|}

%\def\bu{\ensuremath{\mathbf{u}}} 
\def\dH{\ensuremath{\normalfont{\text{d}_\text{H}}}} 
\def\Rad{\ensuremath{\text{\normalfont{Rad}}}} 
\def\tilq{\ensuremath{\widetilde{q}}} 
\def\cS{{\ensuremath{\mathcal{S}}}} 
\def\AUL{{\ensuremath{\normalfont{\text{AUL}}}}} 
\def\Rel{{\ensuremath{\normalfont{\text{Rel}}}}} 
\def\cF{{\ensuremath{\mathcal{F}}}} 
\def\Mis{{\ensuremath{\normalfont{\text{Mis}}}}} 

\def\tilell{\ensuremath{\tilde{\ell}}} 
\def\btilell{\ensuremath{\widetilde{\boldsymbol{\ell}}}} 
\def\tilL{\ensuremath{\widetilde{L}}} 
\def\barJ{\ensuremath{\overline{J}}} 

% 20171016
\def\Corral{\ensuremath{\normalfont{\textsc{Corral}}}\xspace}
\def\cO{{\ensuremath{\mathcal{O}}}} 
\def\tilO{{\ensuremath{\widetilde{\mathcal{O}}}}} 
\def\Eps{\ensuremath{\mathcal{E}}}
\def\bth{\ensuremath{{\boldsymbol{\theta}}}} 
\def\cR{\ensuremath{\mathcal{R}}} 

\def\SUCB{\ensuremath{\normalfont{\text{SUCB}}}}
\def\tr{{\ensuremath{\normalfont{\text{tr}}}}} 

\def\hcL{\ensuremath{\hat\cL}} 
\def\hS{\ensuremath{\hat S}} 
\def\hL{\ensuremath{\hat\L}} 
\def\hLam{\ensuremath{\what{\Lam}}\xspace} 

\def\dsP{\ensuremath{{\mathds P}}}

%- 20180418
\def\cK{\ensuremath{\mathcal{K}}}
\def\nab{\ensuremath{\nabla}}
\def\th{{\ensuremath{\theta}}}

\def\bPhi{{{\boldsymbol \Phi}}} 
\def\bGamma{{{\boldsymbol \Gamma}}} 




%- 20180426
\def\hVp{\ensuremath{\what{\V}_\perp}} 
\def\baru{\ensuremath{\overline{\u}}} 
\def\barv{\ensuremath{\overline{\v}}} 
\def\bbU{\ensuremath{\overline{\U}}} 
\def\bbV{\ensuremath{\overline{\V}}} 
\def\hbS{\ensuremath{\what{\S}}}

\def\sign{\ensuremath{\normalfont{\text{sign}}}} 
\def\Var{\ensuremath{\normalfont{\text{Var}}}}
\def\Om{{\ensuremath{\Omega}}} 

\def\poly{\operatorname{poly}}
\def\Misid{\operatorname{Misid}}
\def\cH{{\ensuremath{\mathcal{H}}}}
\def\hG{\ensuremath{\hat{G}}} 
\def\hg{\ensuremath{\hat{g}}} 
\def\nab{\ensuremath{\nabla}} 

\def\Reward{\ensuremath{\text{Reward}}}
\def\tiltheta{\ensuremath{\tilde{\theta}}} 
\def\tilp{\ensuremath{\tilde{p}}} 

\def\bxi{{{\boldsymbol \xi}}}
\def\bone{{{\mathbf 1}}}

\def\hell{{{\hat\ell}}}

\def\rhoX{{\rho_{\mathcal{X}}}}
\def\Mis{{\text{Mis}}}

%2019
\def\hR{\ensuremath{\widehat{R}}} 
\def\hcF{\ensuremath{\widehat{\cF}}} 
\def\suchthat{\text{ s.t. }}
\def\cd{\cdot}
\def\cc{{\circ}}
\def\hf{\ensuremath{\widehat{f}}} 
\def\bargam{\ensuremath{\overline{\gamma}}} 
\def\tila{\ensuremath{\widetilde{a}}} 
\def\tilmu{\ensuremath{\widetilde{\mu}}}
\def\tilf{\ensuremath{\widetilde{f}}} 
\def\tilcF{\ensuremath{\widetilde{\cF}}} 
\def\barcF{\ensuremath{\overline{\cF}}} 
\def\barf{\ensuremath{\overline{f}}} 
\def\bara{\ensuremath{\overline{a}}} 
\def\barmu{\ensuremath{\overline{\mu}}} 

\newcommand{\FSB}{{\ensuremath{\text{FSB}}}}
\newcommand{\Cr}{{\ensuremath{\text{Cr}}}}
\newcommand{\SE}{{\ensuremath{\text{SE}}}}
\def\IC{{\ensuremath{\normalfont{\text{IC}}}}}
\newcommand{\Fs}{{\ensuremath{\text{Fs}}}}
\newcommand{\barFs}{{\ensuremath{\wbar{\text{Fs}}}}}
\def\rcF{\ensuremath{\mathring{\cF}}} 
\def\rbeta{\ensuremath{\mathring{\beta}}} 
\def\Cf{{\ensuremath{{\normalfont{\text{Cf}}}}}}
\def\barCf{{\ensuremath{\wbar{\text{Cf}}}}}
\def\ralpha{\ensuremath{{\mathring{\alpha}}}} 
\newcommand{\Fb}{{\ensuremath{\text{Fb}}}}
\def\rz{\ensuremath{\mathring{z}}} 

\DeclareMathOperator{\SReg}{{\mathsf{SReg}}}
\DeclareMathOperator{\MisPrb}{{{\mathsf{MisPrb}}}}
\def\SR{{\ensuremath{\text{SR}}}\xspace}
\def\lin{{\ensuremath{\mathsf{lin}}}}
\def\Bernoulli{{\ensuremath{\mathsf{Bernoulli}}}}
\def\lammin{{\lam_{\min}}}

\newcommand{\mytag}[1]{\tag*{$\del{#1}$}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}

\newcommand\msf[1]{{\mathsf{#1}}}
\def\dmu{\dot\mu}

\def\teff{{\ensuremath{t_\mathsf{eff}}}}
\def\sp{{\ensuremath{\mathsf{p}}}}
\def\sq{{\ensuremath{\mathsf{q}}}}

\DeclareMathOperator{\barln}{\overline\ln}% 20210301
\def\erfc{\mathsf{erfc}}
\def\nck#1#2{\begin{pmatrix}
    #1 \\ #2
\end{pmatrix}}

\def\onec#1{\one\cbr{#1}}

\def\tsty{\textstyle}

\newcommand{\normz}[1]{{\norm[0]{#1}}}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

\safedef\tmin{{\min}}
\safedef\tmax{{\max}}


==> sections/def-kjun-v5-shared.tex <==
%--- synctex
\synctex=1
% \pdfoutput=1  % for arxiv submission

%--- prints out an error when the symbol is already defined.
\def\safedef#1{% 
   \ifx#1\undefined
      \expandafter\def\expandafter#1%
   \else
      \errmessage{The \string#1 is defined already}% 
      \expandafter\def\expandafter\tmp
   \fi
}

%--- math better math font
\usepackage{amsthm,amsmath,bbm,amsfonts,amssymb}
\usepackage{dsfont} % require for using \mathds{1}
\usepackage{mathtools}
\usepackage{commath}
\usepackage{eqnarray}
\mathtoolsset{showonlyrefs=false}
\allowdisplaybreaks % This allows breaking multi-line equations

%--- font and spacing
\usepackage{xspace}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[usenames,dvipsnames]{xcolor} % for color names

%--- links
\usepackage{hyperref,url}
%\usepackage{cleveref} % must be loaded after amsthm

%--- floating objects
\usepackage{wrapfig}
\usepackage[export]{adjustbox}
\safedef\imagetop#1{\vtop{\null\hbox{#1}}} % adjusting location of box in table
\usepackage{graphicx,tabularx}
\usepackage{multirow,hhline}% http://ctan.org/pkg/multirow
\usepackage{booktabs}% to use \midrule for drawing a horizontal line in align environment
\usepackage{pbox} % new line in a table cell -- http://tex.stackexchange.com/questions/2441/how-to-add-a-forced-line-break-inside-a-table-cell
%\usepackage{algorithm,algorithmic}

%- for vertical alignment of includegraphics
%- http://tex.stackexchange.com/questions/101858/make-two-figures-aligned-at-top
\usepackage[export]{adjustbox}

%--- etc
%\usepackage{capt-of}
%\newcommand{\fix}{\marginpar{FIX}}
%\newcommand{\new}{\marginpar{NEW}}

\usepackage{enumitem}
%\usepackage{etoolbox}


% define your comment color here
\newcommand{\kwang}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}
\newcommand{\kw}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}
\newcommand{\kj}[1]{{\color{RedOrange}[#1]}}
\newcommand{\ks}[1]{{\color{OliveGreen}Kyoungseok: #1}}
\newcommand{\chicheng}[1]{{\color{blue}Chicheng: #1}}
\newcommand{\fo}[1]{{\color{Violet}[FO: #1]}}
\newcommand{\my}[1]{{\color{ForestGreen}[FO: #1]}}
\newcommand{\gray}[1]{{ \color[rgb]{.6,.6,.6} #1 }}
\newcommand{\blue}[1]{{\color[rgb]{.3,.5,1}#1}}
\newcommand{\tblue}[1]{{\color[rgb]{0,0,1}#1}} % 'the' blue
\newcommand{\grn}[1]{{\color{ForestGreen}#1}}
\newcommand{\org}[1]{{\color{Orange}#1}}
\newcommand{\vio}[1]{{\color{Violet}#1}}
\newcommand{\red}[1]{{\color[rgb]{1,.1,.1}#1}}
\newcommand{\gr}[1]{{\color[rgb]{.8,.8,.8}#1}}

\newcommand{\clb}[1]{{\color{blue}#1}}
\newcommand{\clg}[1]{{\color{green}#1}}
\newcommand{\clr}[1]{{\color{red}#1}}
\newcommand{\clc}[1]{{\color{cyan}#1}}

%---------- setup theorem environment
\usepackage{framed}
\usepackage[most]{tcolorbox}
\definecolor{kjgray}{rgb}{.7,.7,.7}

\newtheoremstyle{kjstyle}
{1ex} % Space above
{\topsep} % Space below
{\itshape} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')

\newtheoremstyle{kjstyle2}
{.0em} % Space above
{.0em} % Space below
{\itshape} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')


\newtheoremstyle{kjstylenoitalic}
{1ex} % Space above
{\topsep} % Space below
{} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')

\tcbset{kjboxstyle/.style={title={},breakable,colback=white,enhanced jigsaw,boxrule=1.3pt,sharp corners,colframe=kjgray,boxsep=0pt,coltitle={black},attach title to upper={},left=.8ex,bottom=.4em}}    

\tcbset{kjboxstylec/.style={title={},breakable,colback=white,enhanced jigsaw,boxrule=1.3pt,sharp corners,colframe=kjgray,boxsep=0pt,coltitle={black},attach title to upper={},before skip=1.5ex,left=.8ex,bottom=.4em,top=0.4em,enlarge top by=-0.3em,enlarge bottom by=-0.3em}}    
%    ,title after break={Lemma \thelemma\ (continued)}}
%}

% \newtheorem{theorem}{Theorem}

% \theoremstyle{kjstyle}\newtheorem{thm}{Theorem}
% \AtBeginEnvironment{thm}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{thm}{\end{tcolorbox}}%
% \theoremstyle{kjstyle}\newtheorem{lem}[thm]{Lemma}
% \AtBeginEnvironment{lem}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{lem}{\end{tcolorbox}}%
% %\theoremstyle{kjstyle}\newtheorem{lem}[thm]{Lemma}
% %\AtBeginEnvironment{lem}{\begin{tcolorbox}[kjboxstyle]}%
% %  \AtEndEnvironment{lem}{\end{tcolorbox}}%
% \theoremstyle{kjstyle}\newtheorem{prop}[thm]{Proposition}
% \AtBeginEnvironment{prop}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{prop}{\end{tcolorbox}}%
% \theoremstyle{kjstyle}\newtheorem{cor}[thm]{Corollary}
% \AtBeginEnvironment{cor}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{cor}{\end{tcolorbox}}%

% \theoremstyle{kjstyle}\newtheorem{defn}{Definition}
% \AtBeginEnvironment{defn}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{defn}{\end{tcolorbox}}%

% \theoremstyle{kjstyle}\newtheorem{ass}{Assumption}
% \AtBeginEnvironment{ass}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{ass}{\end{tcolorbox}}%
% \renewcommand\theass{A\arabic{ass}}

% \theoremstyle{kjstyle}\newtheorem{conj}{Conjecture}
% \AtBeginEnvironment{conj}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{conj}{\end{tcolorbox}}%


% \theoremstyle{kjstyle}\newtheorem{question}{Question}
% \AtBeginEnvironment{question}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{question}{\end{tcolorbox}}%
% % \renewcommand\theass{A\arabic{ass}}

% \theoremstyle{kjstylenoitalic}\newtheorem{remark}{Remark}
% \AtBeginEnvironment{remark}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{remark}{\end{tcolorbox}}%
% \theoremstyle{kjstylenoitalic}\newtheorem{openp}{Open Problem}
% \AtBeginEnvironment{openp}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{openp}{\end{tcolorbox}}%

% \theoremstyle{kjstylenoitalic}\newtheorem{ex}{Example}
% \AtBeginEnvironment{ex}{\begin{tcolorbox}[kjboxstyle]}%
%   \AtEndEnvironment{ex}{\end{tcolorbox}}%

% \theoremstyle{kjstylenoitalic}\newtheorem{prob}{Problem}


%--------------- other ways to create box
\newcommand{\kjunboxold}[1]{\vspace{.5em}\\\fbox{%
    \begin{minipage}{\linewidth}
      \centering #1
    \end{minipage}%
  }\vspace{.5em}}
\usepackage{mdframed}
\usepackage{lipsum}
\definecolor{kjgray}{rgb}{.7,.7,.7}
\makeatletter
\newcommand{\kjunbox}[1]{\vspace{.4ex}
  \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt]
    #1
  \end{mdframed}%
}
\makeatletter
\newcommand{\kjunboxcenter}[1]{\vspace{.4ex}
  \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt,userdefinedwidth=.8\linewidth,align=center]
    %[linecolor=black,innerleftmargin=.4em,innerrightmargin=.4em,userdefinedwidth=.8\linewidth,align=center]
    #1
  \end{mdframed}%
}
\makeatother


%--- to remove the space before paragraph : change 3.25ex to ...
\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0.50ex \@plus 1ex \@minus .2ex}{-1em}%
  {\normalfont\normalsize\bfseries}%
}
\makeatother

%------- this makes a border that covers other part of the equation....
%- https://tex.stackexchange.com/questions/72692/highlight-an-equation-within-an-align-environment-with-color-option
\usepackage[customcolors,shade]{hf-tikz} % after {}, (right, below) and then (left, above) offset... I don't know how it works; done by trial-and-error.
\newcommand{\hll}[2]{\tikzmarkin[set fill color=yellow!30]{#1}(0.02,-.08)(-0.02,0.3)#2\tikzmarkend{#1}}

%--------------------- better paragraph environment
\newcommand{\myparagraph}[1]{\paragraph{[#1]}\mbox{}\\}

%---- useful sometimes
\safedef\horizontalline{\noindent\rule{\textwidth}{1pt} }

%--- better table
\usepackage{tabularx} 
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}

%- hollow
\def\ddef#1{\expandafter\def\csname #1#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDFGHIJKLMNORSTUWXYZ\ddefloop % except for E P V Q

%- c: mathcal
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

%- b: mathbf/boldsymbol
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop  
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{{\boldsymbol{#1}}}}}
\ddefloop abcdeghijklmnopqrtsuvwxyz\ddefloop  % except for bf, which often causes an issue

%- h: hat
\def\ddef#1{\expandafter\def\csname h#1\endcsname{\ensuremath{\hat{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrsuvwxyz\ddefloop % except for 't'
\def\ddef#1{\expandafter\def\csname hc#1\endcsname{\ensuremath{\hat{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname hb#1\endcsname{\ensuremath{\hat{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop % 
\def\ddef#1{\expandafter\def\csname hb#1\endcsname{\ensuremath{\hat{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- t: til
\def\ddef#1{\expandafter\def\csname t#1\endcsname{\ensuremath{\tilde{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefgijklmnpqtsuvwxyz\ddefloop % except for o and h and r
\def\ddef#1{\expandafter\def\csname tc#1\endcsname{\ensuremath{\tilde{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname tb#1\endcsname{\ensuremath{\tilde{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname tb#1\endcsname{\ensuremath{\tilde{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- bar
\def\ddef#1{\expandafter\def\csname bar#1\endcsname{\ensuremath{\bar{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname barc#1\endcsname{\ensuremath{\bar{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname barb#1\endcsname{\ensuremath{\bar{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname barb#1\endcsname{\ensuremath{\bar{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- war: wide bar
\def\ddef#1{\expandafter\def\csname war#1\endcsname{\ensuremath{\overline{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname warc#1\endcsname{\ensuremath{\overline{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname warb#1\endcsname{\ensuremath{\overline{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname warb#1\endcsname{\ensuremath{\overline{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- exceptions
\safedef\tilr{\tilde r}
\safedef\bff{{\boldsymbol f}}
\safedef\hbff{{\hat{\boldsymbol f}}}
\safedef\hatt{\hat{t}}
\safedef\tilo{{\tilde{o}}}
\safedef\tilh{{\tilde{h}}}
\safedef\bell{{{\boldsymbol\ell}}}
\safedef\tell{\ensuremath{\tilde{\ell}}} 
\safedef\btell{\ensuremath{\widetilde{\boldsymbol{\ell}}}} 
\safedef\hell{{{\hat\ell}}}

\safedef\rialpha{\ensuremath{{\mathring{\alpha}}}} 
\safedef\riz{\ensuremath{\mathring{z}}} 
\safedef\ribeta{\ensuremath{\mathring{\beta}}} 

%--- generic shortcuts
\newcommand{\fr}[2]{ { \frac{#1}{#2} }}
\newcommand{\tfr}[2]{ { \tfrac{#1}{#2} }}
\newcommand{\til}[1]{{\ensuremath{\tilde{#1}}}}
\newcommand{\wtil}[1]{{\ensuremath{\widetilde{#1}}}}
\newcommand{\wil}[1]{{\ensuremath{\widetilde{#1}}}}
\newcommand{\wbar}[1]{{\ensuremath{\overline{#1}}}}
\newcommand{\war}[1]{{\ensuremath{\overline{#1}}}}
\newcommand{\what}[1]{{\ensuremath{\widehat{#1}}}}
\newcommand{\wat}[1]{{\ensuremath{\widehat{#1}}}}
\newcommand\msf[1]{{\mathsf{#1}}}
\newcommand{\T}{\top}
\safedef\wed{\wedge}
\safedef\tsty{\textstyle}
\safedef\bec{\because}
\newcommand{\nab}{\nabla}
\safedef\cd{\cdot}
\safedef\cc{{\circ}}
\safedef\la{\langle}
\safedef\ra{\rangle}
\safedef\dsum{\ensuremath{\displaystyle\sum}} 
\safedef\der{\ensuremath{\partial}\xspace}
\safedef\llfl{\left\lfloor} 
\safedef\rrfl{\right\rfloor}  
\safedef\llcl{\left\lceil}  
\safedef\rrcl{\right\rceil}  
\safedef\lfl{\lfloor} 
\safedef\rfl{\rfloor}  
\safedef\lcl{\lceil}  
\safedef\rcl{\rceil}  
\safedef\larrow{\ensuremath{\leftarrow}\xspace} 
\safedef\rarrow{\ensuremath{\rightarrow}\xspace} 
\safedef\sm{{\ensuremath{\setminus}\xspace} }
\safedef\grad{\ensuremath{\mathbf{\nabla}}\xspace}  
\safedef\lt{\left}
\safedef\rt{\right}

%- checkmarks.
\definecolor{mygrn}{rgb}{0,.8,0}
\definecolor{myred}{rgb}{.8,0,0}
\newcommand{\mycm}{\textcolor{myred}{\cmark}}
\newcommand{\myxm}{\textcolor{myred}{\xmark}}

%--- greek
\safedef\sig{\sigma}
\safedef\om{\omega}
\safedef\dt{\delta}
\safedef\gam{\gamma}
\safedef\lam{\lambda}
\safedef\kap{\kappa}
\safedef\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\th{\theta}
\safedef\Lam{\Lambda}
\safedef\Dt{\Delta}
\safedef\Gam{\Gamma}
\safedef\Sig{\Sigma}
\safedef\Th{\Theta} 
\safedef\Om{\Omega}

\usepackage{pgffor}
\safedef\greeksymbols{alpha,beta,gamma,gam,delta,dt,eps,epsilon,zeta,eta,theta,th,iota,kappa,kap,lambda,lam,mu,nu,xi,pi,rho,sigma,sig,tau,phi,chi,psi,omega,om,Gamma,Gam,Delta,Dt,Theta,Th,Lambda,Lam,Pi,Sigma,Sig,Phi,Psi,Omega,Om}
\safedef\greeksymbolsnoeta{alpha,beta,gamma,gam,delta,dt,eps,epsilon,zeta,theta,th,iota,kappa,kap,lambda,lam,mu,nu,xi,pi,rho,sigma,sig,tau,phi,chi,psi,omega,om,Gamma,Gam,Delta,Dt,Theta,Th,Lambda,Lam,Pi,Sigma,Sig,Phi,Psi,Omega,Om} % except for eta

%- prefix b: boldsymbol
\foreach \x in \greeksymbolsnoeta{\expandafter\xdef\csname b\x\endcsname{\noexpand\ensuremath{\noexpand\boldsymbol{\csname \x\endcsname}}}}
\safedef\bfeta{{\boldsymbol \eta}}

%- prefix h, hb: hat, hat bold
\foreach \x in \greeksymbols{\expandafter\xdef\csname h\x\endcsname{\noexpand\ensuremath{\noexpand\hat{\csname \x\endcsname}}}}
\foreach \x in \greeksymbolsnoeta{\expandafter\xdef\csname hb\x\endcsname{\noexpand\ensuremath{\noexpand\hat{\noexpand\boldsymbol{ \csname \x\endcsname}}}}}
\safedef\hbfeta{{\hat{\boldsymbol \eta}}}

%- prefix bar, barb: bar, bar bold
\foreach \x in \greeksymbols{\expandafter\xdef\csname bar\x\endcsname{\noexpand\ensuremath{\noexpand\bar{\csname \x\endcsname}}}}
\foreach \x in \greeksymbolsnoeta{%
\expandafter\xdef\csname barb\x\endcsname{\noexpand\ensuremath{\noexpand\bar{\noexpand\boldsymbol{ \csname \x\endcsname}}}}
}
\safedef\barbfeta{{\bar{\boldsymbol \eta}}}

%- prefix t, tb: tilde, tilde bold
\foreach \x in \greeksymbols{\expandafter\xdef\csname t\x\endcsname{\noexpand\ensuremath{\noexpand\tilde{\csname \x\endcsname}}}}
\foreach \x in \greeksymbolsnoeta{\expandafter\xdef\csname tb\x\endcsname{\noexpand\ensuremath{\noexpand\tilde{\noexpand\boldsymbol{ \csname \x\endcsname}}}}}
\safedef\tbfeta{{\tilde{\boldsymbol \eta}}}

\safedef\dmu{{\dot\mu}}
\safedef\ddmu{{\ddot\mu}}

% %--- space
% \safedef\RR{{\mathbb{R}}}
% \safedef\NN{{\mathbb{N}}}
% \safedef\ZZ{{\mathbb{Z}}}
% \safedef\SS{{\mathbb{S}}}
% \safedef\HH{{\mathbb{H}}} 

%--- math operators
\DeclareMathOperator{\EE}{\mathbb{E}} % ensures the left space is proper (e.g., 2\EE[X])
\DeclareMathOperator{\VV}{\mathbb{V}}
\DeclareMathOperator{\PP}{\mathbb{P}}
\DeclareMathOperator{\QQ}{\mathbb{Q}}
\DeclareMathOperator{\hEE}{\hat{\mathbb{E}}}
\DeclareMathOperator{\Var}{{\text{Var}}}
\DeclareMathOperator{\barln}{\overline\ln}%
\DeclareMathOperator{\tr}{\text{\normalfont tr}}
\DeclareMathOperator{\conv}{\text{\normalfont conv}}

\safedef\clip#1{\wbar{\del{#1}}}
\DeclareMathOperator{\one}{\mathds{1}\hspace{-.1em}}
\safedef\onec#1{\one\cbr{#1}}

% \newcommand{\binom}[2]{{\begin{pmatrix} %- already exists in some package.. (maybe commath)
%     #1 \\ #2
% \end{pmatrix}}}              
\newcommand{\normz}[1]{{\norm[0]{#1}}}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

%-- relationship operators
\newcommand\declareop[3]{%
  \newcommand#1{%
    \mskip\muexpr\medmuskip*#2\relax
    {#3}%
    \mskip\muexpr\medmuskip*#2\relax
}}
\declareop\capprox{1}{{\sr{\const}{\approx}}} % I think 1 means the amount of space.
\declareop\logapprox{1}{{\sr{\mathsf{log}}{\approx}}} % I think 1 means the amount of space.

\newcommand{\lapp}{\mathop{}\!\lessapprox} 
\newcommand{\gapp}{\mathop{}\!\gtrapprox}
\newcommand{\lsim}{\mathop{}\!\lesssim}
\newcommand{\gsim}{\mathop{}\!\gtrsim}

%---- distribution names
\safedef\Bin{\mathsf{Bin}}
\safedef\Uniform{{\mathsf{Uniform}}}
\safedef\Bernoulli{{\ensuremath{\mathsf{Bernoulli}}}}

%--- string
\safedef\kt{{\mathsf{kt}}}
\safedef\mle{{\mathsf{mle}}}
\DeclareMathOperator{\Supp}{{\mathsf{Supp}}}
\safedef\Approx{{\mathsf{Approx}} }
\safedef\denom{{\mathsf{denom}}}
\safedef\eff{{\mathsf{eff}}}
\safedef\Seff{{S_{\mathsf{eff}}}}
\safedef\opt{{\mathsf{opt}}}
\safedef\pes{{\mathsf{pes}}}
\safedef\faury{{\mathsf{faury}}}
\safedef\nice{{\textsf{nice} } } 
\safedef\ErrPrb{{\mathsf{ErrPrb}}}
\safedef\Seg{{\mathsf{Seg}}}
\safedef\COM{\mathsf{COM}}
\safedef\const{\mathsf{const}}
\safedef\wo{{\ensuremath{\mathsf{wo}}}}
\safedef\Top{\mathsf{Top}}
\safedef\Bot{\mathsf{Bot}}
\safedef\Sim{\mathsf{Sim}}
\safedef\TV{\mathsf{TV}}
\safedef\tmin{{\min}}
\safedef\tmax{{\max}}
\DeclareMathOperator{\rank}{{\mathsf{rank}}}
\safedef\kl{{\mathsf{kl}}}
\safedef\err{\mathsf{err}} 
\safedef\logloss{{\mathsf{logloss}}}
\safedef\Ber{{\mathsf{Ber}}}
\safedef\erf{{\text{erf}}}
\safedef\erfc{\mathsf{erfc}}
\safedef\rcF{\ensuremath{\mathring{\cF}}} 
\safedef\Cf{{\ensuremath{{\normalfont{\text{Cf}}}}}}
\safedef\barCf{{\ensuremath{\wbar{\text{Cf}}}}}
\newcommand{\Fb}{{\ensuremath{\text{Fb}}}}
\DeclareMathOperator{\SReg}{{\mathsf{SReg}}}
\DeclareMathOperator{\MisPrb}{{{\mathsf{MisPrb}}}}
\safedef\SR{{\ensuremath{\text{SR}}}\xspace}
\safedef\lin{{\ensuremath{\mathsf{lin}}}}
\newcommand{\FSB}{{\ensuremath{\text{FSB}}}}
\newcommand{\Cr}{{\ensuremath{\text{Cr}}}}
\newcommand{\SE}{{\ensuremath{\text{SE}}}}
\safedef\IC{{\ensuremath{\normalfont{\text{IC}}}}}
\newcommand{\Fs}{{\ensuremath{\text{Fs}}}}
\newcommand{\barFs}{{\ensuremath{\wbar{\text{Fs}}}}}
\safedef\Reward{\ensuremath{\text{Reward}}}
\safedef\poly{\operatorname{poly}}
\safedef\Misid{\operatorname{Misid}}
\safedef\Corral{\ensuremath{\normalfont{\textsc{Corral}}}\xspace}
\safedef\AUL{{\ensuremath{\normalfont{\text{AUL}}}}} 
\safedef\Rel{{\ensuremath{\normalfont{\text{Rel}}}}} 
\safedef\Mis{{\ensuremath{\normalfont{\text{Mis}}}}} 
\safedef\Rad{\ensuremath{\text{\normalfont{Rad}}}} 
\DeclareMathOperator*{\argmax}{arg~max}
\DeclareMathOperator*{\argmin}{arg~min}
\DeclareMathOperator{\diag}{{\text{diag}}}
\DeclareMathOperator{\supp}{{\text{supp}}}
\DeclareMathOperator{\sign}{{\text{sign}}}
\DeclareMathOperator{\KL}{{\mathsf{KL}}}

\safedef\Reg{{\mathsf{Reg}}}
\safedef\Regret{\ensuremath{\normalfont{\text{Regret}}}}
\safedef\Wealth{\ensuremath{\normalfont{\text{Wealth}}}}
\safedef\Active{\ensuremath{\text{Active}}}
\safedef\decomp{\ensuremath{\mbox{decomp}}\xspace}
\safedef\sym{{\ensuremath{\text{Sym}}\xspace}} 
\safedef\suchthat{\ensuremath{\text{ s.t. }}} 


%--- min/max
\newcommand{\hyphen}{{\text{-\hspace{-.06em}}}}
\newcommand\kmax[1]{\mathop{#1\hyphen\max}}
\newcommand\kmin[1]{\mathop{#1\hyphen\min}}

%--- colored checkmarks.
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\cm}{\ding{51}}%
\newcommand{\gyes}{{\color[rgb]{0,.8,0}\cmark}}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\xm}{\ding{55}}%
\newcommand{\rno}{{\color[rgb]{.8,0,0}\xmark}}
\newcommand{\no}{\mbox{\clr{\ding{55}}}}
\newcommand{\yes}{\mbox{\clg{\ding{51}}}}

%--- add equations above or below.
\newcommand{\ubrace}[2]{{\underbrace{#1}_{\textstyle #2}}}
\newcommand{\sr}[2]{ {\stackrel{#1}{#2}} }

%--- parenthesis or symbols with parenthesis
\newcommand{\evt}[1]{\envert{#1}}
\newcommand*{\medcup}{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}}%
\newcommand*{\medcap}{\mathbin{\scalebox{1.5}{\ensuremath{\cap}}}}%
\safedef\bigmid{\,\middle|\,\xspace}
\newcommand{\bmid}{\;\middle|\;}
%- super large parenthesis
\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother

%--- etc.
\safedef\rhoX{{\rho_{\mathcal{X}}}}
\safedef\lammin{{\lambda_{\min}}}
\safedef\elllog{{\ell^{\mathsf{log}}}}

%---- for equationarray
%\arraycolsep=1.4pt
%\def\arraystretch{3}
\def\mytag#1{\hfill\text{(#1)}}


%--------- 23-0415
\safedef\resh{\text{resh}}
\safedef\SVD{\text{SVD}}
\safedef\op{{\text{op}}}
\safedef\sT{{*\T}}


==> sections/intro_old.tex <==
\section{Introduction and Related works}\label{sec:intro}
In many real-world applications, data exhibit low-rank structure. For example, in the Netflix problem~\citep{bennett2007netflix}, the user-movie rating matrix can be well-approximated by a low-rank matrix; in demographic surveys~\citep{udell2016generalized}, the respondents' answers to the survey questions are also oftentimes modeled as a low-rank matrix. 
Motivated by these applications, estimation with low-rank structure is {one of the central themes} in high-dimensional statistics~\citep[][Chapter 10]{wainwright_2019}. 
%widespread 


%Low-rank bandit has garnered significant attention from researchers recently. With the increasing complexity of real-world environments, there is a growing interest in high-dimensional reinforcement learning and bandits, where many features need to be taken into account to make optimal decisions. However, as suggested by \citet{wainwright_2019}, without specific structures to exploit, it is practically impossible to learn effective policies. In response, researchers have proposed various structural assumptions such as sparsity or low-rankness to make the learning problem more tractable. This low-rank bandit model can be applicable to various practical scenarios, such as traveling websites, online advertisements, drug discovery, and clothing websites \citep{lu2021low, jun19bilinear}. 

%based on the past arms and rewards
%low-rank

%\chicheng{The current introduction does not formally introduce the low-rank trace regression problem. I think we need it, so I changed the text below a bit.
%}


We study the low-rank trace regression problem~\cite{tsybakov2011nuclear,rohde2011estimation,hamidi20worst} and the related problem of low-rank linear bandits~\cite{jun19bilinear,lu2021low}. 
In the low-rank trace regression problem, a learner is given a set of measurements $(X_t, y_t)$ that satisfy that $y_t = \inner{\Theta^*}{X_t} + \eta_t$, where $\Theta^*$ is an unknown matrix with rank at most $r\ll \min(d_1, d_2)$, and $\eta_t$ is a zero-mean $\sigma$-subgaussian noise.
The goal is to recover $\Theta^*$ with low error. 
Relatedly, for the low-rank linear bandit problem, a learner sequentially learns to choose arms from a given arm set to maximize reward. 
For each time step $t\in \{1, \cdots, n\}$, the learner chooses an arm $A_t$ from an arm set $\cA\subset \RR^{d_1 \times d_2}$, and receives a noisy reward $y_t = \inner{\Theta^*}{A_t} + \eta_t$, where $\Theta^*$ is a rank-$r$ matrix and $\eta_t$ is $\sigma$-subgaussian noise. The learner's objective is to maximize its cumulative reward, $\sum_{t=1}^n y_t$.
This low-rank bandit model is applicable to various practical scenarios~\citep{natarajan2014inductive,luo17anetwork, jun19bilinear}.
\edit{}{Throughout, we will use $X_t$ for the supervised learning setting and $A_t$ for the bandit setting.}

\edit{}{Unlike previous works \citep{jun19bilinear, lu2021low, huang2021optimal, kang2022efficient, lattimore20bandit}, we assume that all our arms are operator norm-bounded, and the hidden parameter $\Theta^*$ is nuclear norm bounded. This bounding norm assumption parallels the linear model case where one could assume the boundedness of $(\ell_\infty, \ell_1)$ vs $(\ell_2,\ell_2)$ norm of (arm set, hidden parameter) pair. There is no consensus in the community on which one is more reasonable, but the former is standard in sparse linear models as it allows an efficient estimation of the sparse unknown parameter. This is true for the matrix bandits as well. 
}

\begin{assumption}[operator norm-bounded arm set]
\label{assumption:op-bound}
The arm set $\cA$ is such that $\cA \subseteq \cbr{A\in \mathbb{R}^{d_1 \times d_2}: \|A\|_{\op} \leq 1}$. 
\end{assumption}
%expected reward of any arm lies in $[-R_{\max}, R_{\max}]$:
%For any $\Theta$,
\begin{assumption}[Bounded norm on reward predictor]
\label{assumption:nuc-bound}
The reward predictor has a bounded nuclear norm: $\|\Theta^*\|_*\leq S_1$.
\end{assumption}


%\mathsf{tr}(A_t^\top \Theta^*)
 
 To name a few examples, in drug discovery, each $A_t$ represent the outer product $u_t v_t^\T$ of the feature representations of a pair of (drug $u_t$, protein $v_t$), and $\Theta^*$ encodes the interaction between them; in online advertising, each $A_t$ represent {the outer product of the feature representation of } a pair of (user $u_t$, product $v_t$), and $\Theta^*$ models their interactions.
The bandit problem setup naturally induces an exploration-exploitation tradeoff: as the learner does not know the reward predictor matrix $\Theta^*$, she may need to choose arms that are informative in learning $\Theta^*$; on the other hand, since the learner's objective is maximizing the expected reward, it may also be a good idea to choose arms that the learner believes to yield high reward, based on the past observations. 





% should 
%some time steps to figure out the reward
%which is crucial in estimating the reward
%should stop spending too much time steps for exploring $\Theta^*$ 
%such as traveling websites, online advertisements, drug discovery, and clothing websites . 




%with the fact that $\tr{A^\top B} = \inner{\vec(A)}{\vec(B)}$ 
%shown that applying known matrix results
%specialized procedures yield
%too much on the geometry

Early studies on low-rank bandits  \citep{jun19bilinear,lu2021low, jang21improved} have designed bandit algorithms with lower regret than naive approaches that view this problem as a $d_1d_2$-dimensional linear bandit problem~\citep{ay11improved,abe99associative,auer02using, dani08stochastic}. 
However, previous studies lack understandings on the relationship between the geometry of the arm set and regret bounds. 
Usually they assume that a ``nice'' exploration distribution over the arm set is given  \citep{jun19bilinear,lu2021low,kang2022efficient, li2022simple}, or assume that the arm set has some curvature property (e.g., the unit Frobenius norm ball)~\citep{lattimore21bandit, huang2021optimal}. 
Also, some of them rely on subprocedures that are either computationally intractable~\citep[][Algorithm 1]{lu2021low}, or nonconvex optimization steps without computational efficiency guarantees~\citep{lattimore21bandit,jang21improved}; see Appendix \ref{sec:relwork} for more related works.%
\footnote{
  We exclude \cite{kang2022efficient} from our comparison since their regret bounds involve quantities that have hidden dependence on dimensionality; see Appendix \ref{Appendix:counter examples} for details.} 
To bridge this gap, we ask: \textit{can we develop computationally efficient low-rank bandit algorithms that allow generic arm sets and provide guarantees that adapts to the geometry of the arm set?}

\edit{}{It is natural to apply efficient low-rank matrix recovery results for answering this question, since smaller estimation error leads to fewer samples for exploration thus smaller cumulative regret in bandit problems. \citet{keshavan10matrix} provides recovery guarantees for projection based rank-$r$ matrix optimization for matrix completion, and \citet{rohde2011estimation,tsybakov2011nuclear} provide analysis of nuclear norm regularized estimation method for \edit{matrix recovery}{general trace regression}, with~\citet{rohde2011estimation} providing further analysis on the (computationally inefficient) Schatten-$p$-norm penalized least squares method. }
\edit{}{Among these approaches, researchers regarded the nuclear norm penalized least square \cite{rohde2011estimation,tsybakov2011nuclear} as the classic approach and applied this method directly \cite{lu2021low} to achieve state-of-the-art algorithm for the low-rank bandit with a general arm set. Since better estimation leads better bandit algorithm, we are interested in investigating the following question:}
\begin{center}
    \textit{Is there any algorithm that can outperform the classical nuclear norm penalized least squares?}
\end{center}
%of specific arm sets
%\textcolor{red}{
% For example, \citep{li2022simple} and \citep{kang2022efficient} assumed existence of a certain distribution on arms, and treated parameters associated with the arm set geometry as constants and not including them in the order. We find out in many cases these parameters are important variables that are deeply related with dimensionality. We also provide an example where the algorithm of \citet{huang2021optimal} have much higher regret when the arm set is more general than their original setting. Please check Appendix \ref{Appendix:counter examples} for explanations. 
% }

%dependent quantities
% properly
% and estimation methods have been proposed in high-dimensional statistics~\citep{negahban2012unified}in exploit both structures, 
%, which corresponding to the canonical coordinates of the sparse linear bandit

% In this work, we draw inspirations from recent works on high-dimensional sparse linear bandits~\citep{hao2020high, jang22popart} to design efficient low-rank bandit algorithms that exploits the geometry of the arm set. 
% Although 
% sparsity and low-rank structure have strong resemblance in modeling a ``low degree of freedom'' of the underlying estimation target, 
% the key difference lies in that sparse linear models assume the existence of a small number of coordinates that capture sparsity of the underlying $\theta^*$, while the low-rank linear models assume 
% that $\Theta^*$'s row and column spans are low-dimensional subspaces of Euclidean spaces. We investigate the application of improved techniques in sparse linear bandit \citep{jang22popart, hao2020high} derived from the geometry of the arm set in the context of low-rank bandit. Building upon the findings of two previous papers \citep{jang22popart, hao2020high} and the insights from \citet{minsker2018sub}, we propose a novel matrix estimation method \lpopart, and leverage this as an data-efficient exploration procedure to design two efficient low-rank bandit algorithms. 

%and develop two algorithms that leverage this approach.

%we focus on how to analyze the relationship between the arm set geometry and the cumulative regret. There are many similarities between sparse linear bandit and low-rank bandit. Both address the challenge of effectively extracting valuable information from limited observations in high-dimensional settings. 



%\ja{Suggestion 1: arm set geometry - early studies (two) ignored geometry of the arm set. Algorithm that ignores geometry : Online-to-confidence set conversion.}
%\ja{suggestion 2: maybe we can draw inspiration from the sparse linear bandit papers which proved arm-set dependent regret bounds~\citep{hao2020high,jang22popart}}
%\ja{Previous works are mainly focused on Frobenius norm bound, but 'it is bad for some reason' - }
%\subsection{Main contribution}
\begin{table*}
\small
\begin{tabular}{c|c|c|c|c}
   \toprule
   & Regret bound & \makecell{Regret when\\ $\cA = \cB_{\op}(1)$}& \makecell{Regret when\\ $\cA = \cA_{\text{hard}}$}&Limitation
   \\
   \midrule
\makecell{OFUL \\\!\!\citep{ay11improved}}\!\! & $\tilde{O}(d^2\sqrt{T})$ & $\tilde{O}(d^2\sqrt{T})$& $\tilde{O}(d^2\sqrt{T})$& 
   \\
   \makecell{ESTR \\\citep{jun19bilinear}}& $\tilde{O}(\sqrt{\frac{rd T}{\lambda_{\min}(Q(\pi))}}\del{\frac{\lambda_{1}}{\lambda_{r}}}^3)$& -& -&Bilinear
   % \chicheng{For the rows whose regret bound has $\pi$, we may need to explain $\pi$}
   \\
   
   \makecell{$\epsilon$-FALB \\\citep{jang21improved}}& $\tilde{O}(\sqrt{d^3 T})$& - & - &\makecell{Bilinear \& \\Comp. intractable}\\

   \makecell{rO-UCB \\\citep{jang21improved}}& $\tilde{O}(\sqrt{r d^3 T})$& - & - &\makecell{Bilinear \&\\ Requires oracle}\\
   \makecell{LowLOC \\\citep{lu2021low}}& $\tilde{O}(\sqrt{rd^3 T})$&
   $\tilde{O}(\sqrt{rd^3 T})$ & $\tilde{O}(\sqrt{rd^3 T})$& Comp. intractable
   \\
   \makecell{LowESTR \\\citep{lu2021low}}& $\tilde{O}( d^{1/4}\sqrt{r\frac{d \cdot \lambda_{\max}(Q(\pi))}{\lambda_{\min}(Q(\pi))^2} T}\del{\frac{S_{1}}{\lambda_{r}}})$\footnotemark{}&  $\tilde{O}(\sqrt{rd^{5/2} T})$& $\tilde{O}(\sqrt{rd^{9/2}T})$& \\
   %\citet{lattimore21bandit} &$\tilde{O}( d\sqrt{T})$& \xmark  (symmetric bilinear, $\cA=\SS^{d_1-1}$)& $r=1$\\
   %\citet{huang2021optimal}& $\min(\tilde{O}(d\sqrt{r T}/\lambda_{\min}, (rdT)^{2/3})$&\xmark ($\cA=\{ A: \|A\|_F \leq 1\}$)& \\
   \makecell{Lower bound \\\citep{lu2021low}} & $\Omega(rd\sqrt{T})$ & & \\
   \midrule
   LPA-ETC (Algorithm \ref{alg:etc-lowrank-dr}) & $\tilde{O}((S_1 r^2 \ldyad T^2 )^{1/3})$& $\tilde{O}(r^{2/3}d^{2/3} T^{2/3})$& $\tilde{O}(r^{2/3}d T^{2/3})$&\\
   
   LPA-ESTR (Algorithm \ref{alg:estr-lowrank-dr}) & $\tilde{O}( d^{1/4}\sqrt{\ldyad T}\del{\frac{S_1}{\lambda_{r}}}))$& $\tilde{O}(\sqrt{d^{5/2}T})$& $\tilde{O}(\sqrt{d^{7/2}T})$&\\
%   Lower bound (Ours) & $\Omega(r^{1/3} T^{2/3} \cC_{\min}^{-1/3})$ &\\
   \bottomrule
\end{tabular}
\caption{
A comparison between our result and existing results on low-rank bandits with fixed arm sets and 1-subgaussian noise. 
Here, $\lambda_{1}$ and $\lambda_{r}$ are abbreviations of $\lambda_{1}(\Theta^*)$ and $\lambda_{r}(\Theta^*)$, respectively, $Q(\pi)$ is the covariance matrix defined in Eq. \eqref{eq: covariance matrix}, $\cB_{\op}(1)$ is the unit operator norm ball, $\cA_{\text{hard}}$ is a special arm set (See Lemma~\ref{lem: comparison between ldyad and cmin}), and 
$\ldyad$ is an arm set dependent constant defined in Eq. \eqref{eq: def of blambda}.
When $\cA \subseteq \cB_{\op}(1)$,  we have $\ldyad = \Omega(d^2)$ and $\lambda_{\min}(Q(\pi)) = O(\frac{1}{d})$, $\forall \pi \in \cP (\cA)$.
For the third and fourth columns, we set $\pi$ to be the most favorable sampling distribution for prior results as they did not specify the sampling distribution $\pi$ but assumed favorable conditions to hold.
% Since $\ldyad \leq \frac{d}{\lambda_{\min}(Q(\pi))}$ holds for any sampling distribution $\pi \in \cP (\cA)$, \last{\textbf{our LPA-ESTR always outperforms previously known low-rank bandit algorithms, especially LowESTR}.
% Further, compared with the best $\lam_{\min}(Q(\pi))$-free guarantee, which attains $\tO(rd^3 T)$, LPA-ETC attains an improved regret when the dimension is relatively large compared to $T$, i.e., $T< O\del{\frac{d^9}{r\ldyad^2}}$. % compared to other low-rank algorithms. 
% used favorable assumptions and regarded existence of such sampling distribution $\pi$ as their assumption.
% }
%Note that most of the prior works assume Frobenius norm bound of $\Theta^*$, so in the setups of the prior works, $\lam_\tmin \leq 1/\sqrt{r}$ but for us we assumed nuclear norm bound of $\Theta^*$ so it is $\lambda_{\min} \leq 1/r$.
%\chicheng{(1) Can we include the lower bound here? (2) For Kang et al, leave a footnote that ``see Section~\ref{sec:relwork} for detailed explanations'' (3) For Huang et al, they have another result on arm set $\cA = \cbr{ u v^\top: u \in \SS^{d_1-1}, v \in \SS^{d_2-1} }$ - they only present this implicitly in their Remark 3.2. Perhaps also include that result in this table?
%}
$S_1$ is an upper bound for  $\|\Theta^*\|_1$, see Assumption \ref{assumption:nuc-bound}.
}


\label{table:comparison}
%\ks{1) Erase all the bilinear results from the third column. 2) For LowESTR and Ours, try to use $S_1$ for demonstration. 3) Change $Sig(Q)$ to $\lambda_{max} (Q(\pi))$, and change all $C_{min}$ to $\lambda_{\min}(Q(\pi))$. 4) Add footnote for the explanation of modification.5) Never worse than LowESTR. 6) Add column of hard case. 7) Cmin, unify to unscripted version. 8) Our algorithm: give name as LPA-ETC, LPA-ESTR }
\end{table*}

% \ks{To answer these items,
% \begin{itemize}
%     \item 1,3) When I wrote this table, most of the results are based on $\|a\|_F \leq 1$, frobenius norm bounded. I need more detailed analysis, but basically I think we can simply multiply $\min(d_1, d_2)$ for all elements in naive approach since $\|a\|_F \leq \sqrt{\min(d_1, d_2)}\|a\|_{op}$ 
%     \item 2) Yes, Lu has two upper bound, I will fix it.
%     \item 4, 5) I think we need to talk about it.
%     \item 6) As far as I know, the only lower bound that I know is of \citep{lu2021low}, $\Omega(rd\sqrt{T})$.
% \end{itemize}
% }


% with dimensional improvements

%We also find out that the traditional convex optimization is enough for finding sampling distribution to control the error bound of \lpopart.

%This approach is useful in the settings where the learner can control the sampling distribution, such as bandits. 

In this paper, we make meaningful progress in high-dimensional low-rank regression and low-rank
bandits, which provides algorithms with arm-set-adaptive exploration and regret analyses for general operator-norm-bounded arm sets. 

\ks{move assumptions above to here.}

\textbf{First,} 
% drawing inspiration from recent works on high-dimensional sparse linear bandits~\citep{hao2020high,jang22popart}, 
under the additional assumption that the measurement distribution $\pi$ is accessible to the learner,
we propose a novel and computationally efficient low-rank estimation method called \lpopart (Low-rank POPulation covariance regression with hARd Thresholding) and prove its estimation error guarantee (Theorem~\ref{thm:wlpopart}) as follows:
%which enjoys an improved operator-norm-based estimation error bound and applicable for general arm sets. \kj{can we say that we, for the first time, provide a precise regret bound that scale with the geometry of the arm set rather than leaving it unspecified like prior works did?} 
% Specifically, the estimation error guarantee (Theorem~\ref{thm:wlpopart}) is of the form 
\[ 
\| \hat{\Theta} - \Theta^* \|_{\op}
\leq 
\tilde{O}\del{ \sigma \sqrt{\frac{B(Q(\pi))}{n_0}} },
\]
where $n_0$ is the number of samples used, and ${B(Q(\pi))}$ (see Eq.~\eqref{eq: optimization of blambda}) is a quantity that depends on the covariance matrix $Q(\pi)$ of the data distribution $\pi$ over the measurement set $\cA$. 
We show that the recovery guarantee of \lpopart is not worse and can sometimes be much better than the classical nuclear norm penalized least squares method~\citep{tsybakov2011nuclear} (see Section \ref{sec:new analysis}).
%the measurement set $\cA$
%arm-set dependent parameter that captures the geometry of


%adaptive compressed sensing and
\textbf{Second,} motivated by the
operator norm recovery bound of \lpopart, we propose a design of experiment objective $B(Q(\pi))$ for finding the sampling distribution that minimizes the error bound of \lpopart. This is useful in settings when we have control on the sampling distribution, such as low-rank linear bandits, the focus of the latter part of this paper.
Applying the recovery bound to the optimal design distribution, we obtain a recovery bound of 
\[ 
\| \hat{\Theta} - \Theta^* \|_{\op}
\leq 
\tilde{O}\del{ \sigma \sqrt{\frac{ \ldyad }{n_0}} },
\]
where $B_{\min}(\cA) := \min_{\pi \in \Delta(\cA)} B(Q(\pi))$ depends on the geometry of the measurement set $\cA$. For example, letting $d := \max\{d_1, d_2\}$, we have $\ldyad = \Theta(d^2)$ and $\Theta(d^3)$ when $\cA$ is the unit operator norm ball and unit Frobenius norm ball, respectively.
%arm
Moreover, optimizing our experimental design criterion is computationally tractable. 
In contrast, many prior works on low-rank matrix recovery require finding a sampling distribution that satisfies properties such as restricted isometry property and restricted eigenvalue \citep{hamdi2022low, tsybakov2011nuclear, wainwright_2019} - all these are computationally intractable to compute or verify and thus hard to optimize \citep{Bandeira_2013, juditsky2011verifiable}, which is even harder when the measurements must be limited to an arbitrarily given set $\cA$.
% \chicheng{check ``restricted strong convexity''}
% \kj{check if compatibility constant is a concept that appears in the low-rank matrix recovery literature.}
% \chicheng{In the NeurIPS rebuttal, we mentioned the reference ``Bandeira et al, Certifying the Restricted Isometry Property is Hard, 2012.'' 
% Are there references specific to low-rank matrix regression?}
% \chicheng{Incoherence is actually computationally tractable to verify?
% See also \url{https://link.springer.com/content/pdf/10.1007/s10107-010-0417-z.pdf} for some other sufficient condition}
%{the experimental design}
%Many of the previous studies \citep{kang2022efficient,jun19bilinear, li2022simple} are based on the works from the matrix recovery,
%\kj{now that I think, it is also natural to consider all these assumptions for matrix recovery (coherence, RIP, etc.; see also ``On Low-rank Trace Regression under General Sampling Distribution''). but the story will be just like popart -- we cannot optimize them.  Our contribution is that our criteria is computable and thus we can optimize it.}; 
%bounded arm set, and $\cC_{min} (\cA)=1/d^2$ when $\cA$ is
%respectively, when 
% := \max_{\pi \in \Delta(\cA)} \lambda_{\min} \EE_{A \sim \pi}[\vec(A) \vec(A)^\top]
%\edit{}{
%This is the first algorithm that provides a precise regret bound that scale with the geometry of the arm set rather than leaving it unspecified like prior works \citep{jun19bilinear,lu2021low,kang2022efficient}.
%Note that many recent works on low-rank bandits assume that a nice ``explorative'' distribution over the arm is given apriori~\citep{kang2022efficient,jun19bilinear, lu2021low, li2022simple}.
%In contrast, our \lpopart provides a principled way to obtain a explorative distribution that yield sharp estimation guarantees.}

\textbf{Finally, }using \lpopart, we propose two computationally efficient and arm set geometry-adaptive algorithms, for low-rank bandits with general arm sets:

% Since $\ldyad \leq \frac{d}{\lambda_{\min}(Q(\pi))}$ holds for any sampling distribution $\pi \in \cP (\cA)$, our LPA-ESTR always outperforms previously known low-rank bandit algorithms, especially LowESTR.
% Further, compared with the best $\lam_{\min}(Q(\pi))$-free guarantee, which attains $\tO(rd^3 T)$, LPA-ETC attains an improved regret when the dimension is relatively large compared to $T$, i.e., $T< O\del{\frac{d^9}{r\ldyad^2}}$.
\begin{itemize}
\item Our first algorithm, LPA-ETC (LowPopArt-Explore-Then-Commit; Algorithm~\ref{alg:etc-lowrank-dr}), leverages the classic explore-then-commit strategy to achieve a regret bound of $\tilde{O}((S_1 r^2 \ldyad T^2)^{1/3})$ (Theorem~\ref{thm:etc regret bound}). 
Compared with the state-of-the-art low-rank bandit algorithms that {allow generic arm sets}~\citep{jun19bilinear,lu2021low} that guarantees a regret order $\tilde{O}(\sqrt{rd^3T})$, Algorithm~\ref{alg:etc-lowrank-dr}'s guarantee is smaller when {$T \ll O( \frac{d^9}{\ldyad^2 r})$} (see Remark~\ref{rem:etc-improve} for a more precise statement). 

%for variable selection 
\item Our second algorithm, LPA-ESTR (LowPopArt-Explore-Subspace-Then-Refine; Algorithm~\ref{alg:estr-lowrank-dr}), works under the extra condition that the nonzero minimum eigenvalue of $\Theta^*$, denoted by $\lambda_{\min}$, is not too small.
% This is analogue to the ``minimum signal condition'' exploited in sparse linear bandits~\citep{hao2020high,jang22popart}. 
Algorithm~\ref{alg:estr-lowrank-dr} uses the Explore-Subspace-Then-Refine (ESTR) framework~\citep{jun19bilinear} and achieves a regret bound of $\tilde{O}( \sqrt{d^{1/2}\ldyad T}S_1 /\lambda_{\min}))$ (Theorem~\ref{thm:estr bound}). %\chicheng{Define $S_1$ here -- something like ``where $S_1$ is an upper bound of .. ''}
LPA-ESTR gives a strictly better regret bound than previously-known computationally efficient algorithms.
For example, compared to LowESTR \citep{lu2021low}, the regret of our LPA-ESTR algorithm makes not only a factor of $\sqrt{r}$ improvement, but also the dependence on the arm set dependent quantity from $\frac{d \lambda_{\max}(Q(\pi))}{\lambda_{\min}(Q(\pi))^2}$ to $\ldyad$; we show that the latter is never larger than the former and that the latter can be a factor of $d$ smaller than the former (Lemma \ref{lem: comparison between ldyad and cmin}). 

\item \edit{}{Both of our algorithms work for general arm sets, unlike many other low-rank bandit algorithms tailored for specific arm sets \cite{katariya17bernoulli,trinh2020solving, kotlowski19bandit, huang2021optimal,lattimore21bandit}.}
%When $\cA$ is the {unit operator norm ball}, compared with the regret guarantee of state-of-the-art low-rank bandit algorithms that also assumes minimum eigenvalue condition~\citep{jun19bilinear,lu2021low} (which is $\tilde{O}( \sqrt{rd^3 T}/\lambda_{\min})$), our regret bound $\tilde{O}( r^{1/4}d^{5/4}T^{1/2}/\lambda_{\min}))$  is lower. 
\end{itemize}
We compare our regret bounds with existing results in Table~\ref{table:comparison}, which showcase how our arm set-dependent regret bounds improve upon prior art in specific arm sets.
We also make a meticulous examination of arm set-dependent constants on regret analysis from previous results, which we believe will help future studies.
\footnotetext{Our bound here is a $d^{1/4}$ factor larger from the original paper since our setting is operator norm bounded action set, which is different from their Frobenius norm bounded action set. For details, see Appendix \ref{appsubsec:d14 modification}. }


%Commented out at 231009
% \textbf{Finally,} we prove a minimax regret lower bound of $\Omega(r^{1/3} T^{2/3} \cC_{\min}(\cA)^{-1/3})$ for low-rank bandits (Theorem~\ref{thm:lower-bound-lr}) in a small-data regime where $T \in [r^2 d^2 , d^4]$. This shows that the regret guarantee of Algorithm~\ref{alg:etc-lowrank-dr}'s dependence on $\cC_{\min}(\cA)$ is fundamental: any attempt in removing the dependence on $\cC_{\min}(\cA)$ in  Theorem~\ref{thm:lower-bound-lr} will come at a price of having a higher dependence on other parameters (e.g. $d$ or $T$).
% It does not contradict with traditional $\sqrt{T}$ regret bounds such as OFUL\citep{ay11improved} or SupLinRel\citep{auer02using} since $T<d^4$. Our upper bound is sublinear as soon as $T \ge (dr)^2$ for favorable arm sets (i.e., $C_\tmin(\cA) = \Theta(d)$).







%\kj{we need to guard against the question of `hey, you are saying the lower bound is of order $T^{2/3}$?' Also, `wait, you can get $\sqrt{d^4 T}$ by flattening out the matrices to vectors, so isn't this a contradiction?'}

%\kj{we can also emphasize: For arm sets whose cardinality is $\Omega(e^{d^2})$, both SupLinRel and OFUL reduction will have a bound of $\sqrt{d^4 T}$, which means that we do not enjoy any guarantee during $T\le d^4$. Our upper bound is sublinear as soon as $T \ge (dr)^2$ for favorable arm sets (i.e., $C_\tmin(\cA) = \Theta(d)$. ``small-data'' regime.}


%with a fixed arm set
% Our algorithms have the following advantages:
% \begin{itemize}
% \item \textbf{Dimensional improvement (Algorithm \ref{alg:etc-lowrank-dr}, \ref{alg:estr-lowrank-dr}):} 

%Traditionally, there have been many attempts to reduce regret bound by focusing on the number of samples, $T$. However, as high dimensionality is often applied in real-life situations, we have attempted a different approach to reduce the order of the $d$, the dimensionality coefficient. As a result, we have discovered a new algorithm that shows a lower dimensional dependency. 
% Especially, our algorithm shows better regret bound than previous general low-rank bandit algorithms (\citep{jun19bilinear,lu2021low}) when $T \ll O(\cC_{\min}^2 d^7/r)$ (Remark~\ref{rem:etc-improve}). Note that there exists a case where $\cC_{min} (\cA)=1/d$ when $\cA$ is operator norm bounded arm set, and $\cC_{min} (\cA)=1/d^2$ when $\cA$ is Frobenius norm bounded arm set. 
% \item \textbf{Generality (Algorithm \ref{alg:etc-lowrank-dr}, \ref{alg:estr-lowrank-dr}):} Recently, several algorithms have been published that use the geometric symmetry of arm sets to achieve significantly improved results \citep{lattimore21bandit, huang2021optimal}. However, these algorithms rely heavily on perfect symmetry and are difficult to apply to more general arm sets. In contrast, our algorithm provides a general result for operator norm bounded arm sets.
% \item \textbf{Independence from the minimum eigenvalue of $\Theta^*$ (Algorithm \ref{alg:etc-lowrank-dr}):} Many of the previous studies depend on the minimum eigenvalue of $\Theta^*$ since their algorithms depend on the decomposition result of SVD. It was counter-intuitive in the multi-armed bandit sense that usually the arms with low reward affects less on the regret upper bound analysis, while the previous low-rank bandit algorithms are being dramatically affected by the size of the minimum eigenvalue. Naturally, those minimum eigenvalue conditions usually induce additional assumption on the minimum eigenvalue or the conditional number. On the other hand, using our genuine thresholding approach, we were able to get a successful regret upper bound analysis without the minimum eigenvalue term. 
% \chicheng{I view the minimum singular value condition for $\Theta$ for low-rank bandits as in parallel to the minimum magnitude condition for $\theta$ for sparse bandit. 
% Recall that in our PopArt paper, we had two algorithms: one for the general assumption-free setting, the other for the setting that requires minimum signal condition. 
% Therefore, a possible organization of this paper is also like this, where we present separate algorithms for these two settings.
% }

%\end{itemize}

%\ks{Write down Algorithm 2 advantages}


==> sections/main_algorithm.tex <==

\section{\textsf{ LowPopArt} - a new exploration and estimation algorithm for low-rank bandits}

%\chicheng{I think this section can benefit from a factorization of the algorithm into two parts: one is a Warm-PopArt like procedure which focuses only on estimating $\Theta$, the other is the usual explore-then-commit procedure. This gives the benefit that the first procedure can be reused in the next section.}

% \chicheng{
% Recall: 
% \[
% F(\pi)
% = 
% \max 
% \del{
% \max_{u \in \mathbb{S}^{d_1-1}} \sbr{ \sum_{i=1}^{d_2} \ve(u \otimes e_i)^\top Q^{-1} \ve(u \otimes e_i) }
% ,
% \max_{v \in \mathbb{S}^{d_2-1}} \sbr{ \sum_{i=1}^{d_1} \ve(e_i \otimes v)^\top Q^{-1} \ve(e_i \otimes v) }
% }
% \]
% We could have set this as our experimental design criterion. 
% But admittedly this is much less cleaner than
% \[
% G(\pi)
% = 
% \max_{u, v \in \mathbb{S}^{d_1-1} \times \mathbb{S}^{d_2-1}} \sbr{ \ve(u \otimes v)^\top Q^{-1} \ve(u \otimes v) }
% \]
% (and we know that $F(\pi) \leq \max(d_1, d_2) G(\pi)$.)
% }

% \ks{TODO: first, check the $R_0$ dependency, and fix the sentences based on the Warm-LowPopArt}
% \ks{TODO: Try to move all the proofs to Appendix to minimize the logical error. }
% \chicheng{Comparison with nuclear-norm-penalized least squares recovery error~\cite{tsybakov2011nuclear}. (similar to what we did in the PopArt paper, that we compare with Lasso) $1/\sqrt{\cC_{\min}}$ is better than $1/\cC_{\min}$.
% This, as we will see, helps get a sharper regret guarantee in low-rank bandits.}

Our main algorithmic tool for designing the bandit algorithm is the following low-rank matrix estimation algorithm Low-rank Population Covariance regression with hARd Thresholding (Algorithm \ref{alg:lowPopart}), abbreviated as LowPopArt. Initially, it calculates an $E$-optimal experimental design distribution $\pi$~\citep{fedorov2013theory}, then samples its action based on the distribution $\pi$ and records the outcomes.
This choice of experimental design distribution is inspired by the sparse linear bandit literature~\citep{hao2020high,jang22popart}. 
Next, it computes the estimation of \citet[Corollary 3.1]{minsker2018sub}, which symmetrizes the original matrix and computes the Catoni function for each eigenvalues (Definition \ref{def:matrix catoni}). We call it as $\Theta_1$. 
We note that Minsker's estimator has also been used in~\cite{kang2022efficient}, although over a different set of samples induced by certain score functions. 
Run SVD on $\Theta_1$ and zeroing out all the singular values smaller than the threshold $\tilde{O}\del{ \sqrt{\frac{(d_1 + d_2)}{n_0 \cC_{\min}} } }$, which is referred as $\hat\Theta$. 

\begin{algorithm}
\caption{Low-rank PopArt}
\begin{algorithmic}[1]
\STATE Input: action set $\cA$, sample size $n_0$, pilot estimator $\Theta_0$ and pilot estimation error bound $R_0$, such that  $\max_{A \in \cA} \abs{ \inner{\Theta_0 - \Theta}{A} } \leq R_0$. 

%regularization parameter $\nu$
\STATE Find 
\begin{equation}
\pi^\star = 
\argmax_{\pi \in \Delta(\cA) } 
\lambda_{d_1 d_2}(Q(\pi))
\label{eqn:expt-design}
\end{equation}

where $Q(\pi) = \EE_{a \sim \pi} \sbr{ \ve(a) \ve(a)^\top }$. Denote by $\cC_{\min}$ the optimal objective function.
\FOR{$t=1,\ldots,n_0$}
\STATE Take action $A_t \sim \pi^\star$, and receive reward $Y_t = \inner{\Theta^*}{A_t} + \eta_t$
\ENDFOR
\STATE
%\chicheng{I think the (inefficient) procedure below for estimating $\Theta$
%is now superceded by our effcient algorithm inspired by~\cite{minsker2018sub}?}
    \[
    \Theta_1    
    =     \Theta_0    +    
    (\frac{1}{n_0 \nu} \sum_{i=1}^{n_0} 
    \psi\del{ \nu \cH\del{ \reshape\del{ Q(\pi)^{-1} (Y_i - \inner{\Theta_0}{X_i}) \ve(X_i) } } }  )_{12}    \]
    where $\nu = 
\frac{1}{\sigma + R_0} \sqrt{\frac{2\cC_{\min}}{d n_0 }\ln \frac{2d}{\delta}}$, and  $(M)_{12}$ refers to the shorthand of $M_{1:d_1, d_1+1:d_1+d_2}$ for any $M\in \RR^{(d_1 + d_2)\times (d_1 + d_2)}$

% \FOR{$(u,v) \in \cN(d, \frac14) \times \cN(d, \frac14)$} 
% \STATE Let $\hat{f}_{u,v} = \catoni( (u \otimes v)^\top \del{ Q(\pi^\star)^{-1} \tilde{A}_t (Y_t - \inner{A_t}{\tau}) + \tau}, t \in (n_1, n_2]) $
% \ENDFOR

% \STATE Let 
% \[ 
% \Theta_1 = \argmin_{\Theta} \max_{u,v \in \cN(d, \frac14) \times \cN(d, \frac14)} 
% \abs{ u^\top \Theta v - \hat{f}_{u,v} }
% \]

%\STATE Let $\tilde{\theta} = \frac{1}{n_2} \sum_{t=n_1+1}^{n_1+n_2} \del{ Q(\pi)^{-1} \tilde{A}_t (Y_t - \inner{A_t}{\tau}) + \tau } \in \RR^{d_1d_2}$ (a vector), and let $\hat{\Theta} \in \RR^{d_1 \times d_2}$ be the rearranged version of $\tilde{\theta}$.
%\Theta_1 = 
\STATE Let $U_1 \Sigma_1 V_1^\T$ be $\Theta_1$'s SVD. Let $\tilde{\Sigma}_1$ be a modification of 
$\Sigma$ by zeroing out its diagonal entries that are smaller than 
$    \sqrt{\frac{\del{ 2(d_1 + d_2)\ln \frac{2(d_1 +d_2)}{\delta} } }{\cC_{\min}n_2}}$. 
%_{n_1+n_2}
\STATE Output: Estimation $\hat\Theta = U_1 \tilde{\Sigma}_1 V_1^\top$. 
\end{algorithmic}
\label{alg:lowPopart}
\end{algorithm}

%need to emphasize
We note that all the operations in Algorithm \ref{alg:lowPopart} can be done efficiently. The first computational part is the optimization in Line 2, minimum eigenvalue optimization, and it is known to be a convex optimization \cite{hao2020high}, so one can use the traditional tools such as CVXPY in Python to optimize the value given the action set. The second computationlly heavy step is Line 6, the first estimation. However, it only involves the element-wise computation and matrix product, once for each timestep $n_0$, so we can say it takes $\tilde{O}((d_1+d_2)^2 n_0)$ computational complexity. Lastly, it also involves SVD computation in Line 7, but it only calls SVD once, so it takes $O((d_1 + d_2)^3)$ order of computation. 
